Towards Optimal Use of Exception Handling Information for Function Detection

Function entry detection is critical for security of binary code. Conventional methods heavily rely on patterns, inevitably missing true functions and introducing errors. Recently, call frames have been used in exception-handling for function start detection. However, existing methods have two problems. First, they combine call frames with heuristic-based approaches, which often brings error and uncertain benefits. Second, they trust the fidelity of call frames, without handling the errors that are introduced by call frames. In this paper, we first study the coverage and accuracy of existing approaches in detecting function starts using call frames. We found that recursive disassembly with call frames can maximize coverage, and using extra heuristic-based approaches does not improve coverage and actually hurts accuracy. Second, we unveil call-frame errors and develop the first approach to fix them, making their use more reliable.

==> new-design.tex <==
\section{Re-designing Exception Handling}
As we aforementioned, removing symbol tables of binaries, in fact, fail to protect binaries from security analysis. 
Eh\_frame section in stripped binary provides large function information which has a huge overlap with those used for binary security analysis.
We hereby propose to redesign exception handling.







==> related.tex <==
\section{Related Works}
\label{sec:related}

In this section, we discuss the research closely related to ours, including function detection and \ehf related research. In addition, one of \tool's major goals is to provide a high level of reliability. Another line of research with a similar goal is formal method based binary analysis. 

\subsection{Function Detection} 
We have discussed most of the general solutions of function detection in \S~\ref{sec:bcg-ehf}. In this section, we discuss another related but non-covered point: using \ehf to help function detection.

Besides \tool, \ghidra~\cite{ghidra_org} and \angr~\cite{shoshitaishvili2016sok} also leverage information from \ehf to help their function detection. However, they use \ehf in a completely different manner from \tool. To be specific, they first perform recursive disassembly and pattern-based matching to recover most of the functions, and then scan through \ehf to identify other function starts. When conflicts arise, they do not prioritize \ehf. In short, they use \ehf to complement the other, often unreliable, approaches. To the contrary, \tool considers \ehf as the major source of information and builds reliable approaches on top of \ehf to detect functions. As demonstrated and reasoned by our evaluation in \S~\ref{sec:eval}, \tool significantly outperforms the two tools in both coverage and precision and more importantly, maintains high reliability. 

\subsection{Research on EH\_Frame} Besides function detection, there are other types of research related to \ehf. Oakley and Bratus~\cite{oakley2011exploiting} exploit \ehf to hijack the control flow without manipulating the run-time data. Technically, they modify data in the \ehf section such that the execution can be diverted for malicious goals (\eg running bash shell) during exception handling. To the contrary, Bastian \etal~\cite{bastian2019reliable} investigate the design problems of \ehf. They unveiled a list of limitations related to \ehf tables, which can raise bugs that hard to be detected and become a bottleneck for time-sensitive program analysis tools. The authors also explored techniques to validate \ehf, synthesize \ehf, and incorporate \ehf into assembly code. 

%While these work
%aims to discuss the attack and defense about \ehf and the DWARF-based
%unwinding, our work focuses on utilizing the information in
%\ehf section to identify function bodies in binary code.

\subsection{Formal Verification for Binary Analysis} Recent research has brought formal methods for binary analysis, producing results with theoretical correctness. For instance, Dasgupta~\etal~\cite{dasgupta2019complete} formally model the non-deprecated, sequential user-level instructions of the x86-64 Haswell architecture. The models can be used for semantic representation in binary disassembly. In addition, \jakstab~\cite{kinder2010precise} develops abstract interpretation that performs VSA to compute an over-approximation of targets of indirect branches, improving the correctness of disassembly. While these works have a different goal from \tool, they can greatly benefit \tool. For instance, \tool can leverage these two works to help its recursive disassembly and therefore, gain an even better guarantee of correctness.





==> scratch.tex <==

\begin{figure*}[!t]
\vspace{-0.1in}
\centering
        \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
          \includegraphics[width=0.25\textwidth, height=4.8cm]{Figure/SourceCode.pdf}
          &
          \includegraphics[width=0.3\textwidth, height=4.8cm]{Figure/AssemblyCode.pdf}
           &
          \includegraphics[width=0.45\textwidth, height=4.9cm]{Figure/Stack.pdf}
        \\
        {\scriptsize (a) Source Code Example}
        &
        {\scriptsize (b) Assembly Code Example}
        &
        {\scriptsize (c) Stack Example}
        \end{tabular}
        \vspace{-0.1in}
       \caption{\small \label{fig:stack-example} Process of unwind stack}
\end{figure*}


% \begin{figure}[t!]
% \begin{minipage}[t]{0.52\textwidth}
% \includegraphics[width=\textwidth]{Figure/Stack.pdf}
% \vspace{1em}
% \end{minipage}
% \hfill
% \end{figure}
% \begin{figure}[t!]
% \begin{minipage}[t]{0.40\textwidth}
% \includegraphics[width=\textwidth]{Figure/AssemblyCode.pdf}
% \vspace{1em}
% \end{minipage}
% \hfill
% \end{figure}

% % DWARF format and unwinding
% Unwind information on modern UNIX-like system is stored in DWARF
% format. On x86\_64 architecture, \texttt{\%rbp} register is generally
% used as a frame pointer to help getting stack traces in the debugger.
% However, the corresponding design has significant overhead. One
% general-purpose register is hold all the time. Accordingly, as x86-64
% ABI suggested, DWARF debug information has been applied to free the
% register used as frame pointer.


\add{(Basics about main start and caller/callee functions)}
The program executes from main function as shown in
\ref{fig:stack-example}. If we analyze in assembly language, <\_start>
function is the real start point of the program execution. Address of
main function will be pass as an argument to \_\_libc\_start\_main.
\_\_libc\_start\_main function will then call main() function with
appropriate argument. The return address of the caller function will
be saved into the stack when program call another function. This is
necessary because the saved return address will guide program return
back to caller function when callee function finish execution.
Accordingly, the return address of <\_\_libc\_start\_main> will be
saved as the first record in the stack. Likewise, when program call
buz() in main(), another stack information will be recorded which
contains the return address of main().


% \begin{figure*}%[ht]
%   \centering
%     \begin{subfigure}[t]{0.25\textwidth}
%     \centering
% \begin{lstlisting}[numbers=none]
% int division(int a, int b)
% {
%   if( b == 0 ) {
%     throw "Division by zero!";
%   }
%   return (a/b);
% }

% int f(int a, int b)
% {
%   int x = a + 10;
%   int y = b;
%   return division(x, y);
% }
% \end{lstlisting}
%     \caption{The source code of function \texttt{f}.}
%     \label{fig:sub1}
%   \end{subfigure}
%   ~
%   \begin{subfigure}[t]{0.35\textwidth}
%     \centering
% \begin{lstlisting}[numbers=none,language={[x86masm]Assembler}]
% 00000968 <_Z1fii>:
% 968: push   ebp
% 969: mov    ebp,esp
% 96b: sub    esp,0x18
% 96e: call   b07 <__x86.get_pc_thunk.ax>
% 973: add    eax,0x162d
% 978: mov    eax,DWORD PTR [ebp+0x8]
% 97b: add    eax,0xa
% 97e: mov    DWORD PTR [ebp-0x10],eax
% 981: mov    eax,DWORD PTR [ebp+0xc]
% 984: mov    DWORD PTR [ebp-0xc],eax
% 987: sub    esp,0x8
% 98a: push   DWORD PTR [ebp-0xc]
% 98d: push   DWORD PTR [ebp-0x10]
% 990: call   91d <_Z8divisionii>
% 995: add    esp,0x10
% 998: leave  
% 999: ret
% \end{lstlisting}
%     \caption{The assembly code of function \texttt{f}.}
%     \label{fig:sub2}
%   \end{subfigure}
%   ~~~~~
%   \begin{subfigure}[t]{0.3\textwidth}
%     \centering
% \begin{lstlisting}[]
% 00000074 0000001c 00000078 FDE 
%   cie=00000000 pc=00000968..0000099a
% DW_CFA_advance_loc: 1 to 00000969
% DW_CFA_def_cfa_offset: 8
% DW_CFA_offset: r5 (ebp) at cfa-8
% DW_CFA_advance_loc: 2 to 0000096b
% DW_CFA_def_cfa_register: r5 (ebp)
% DW_CFA_advance_loc: 46 to 00000999
% DW_CFA_restore: r5 (ebp)
% DW_CFA_def_cfa: r4 (esp) ofs 4
% DW_CFA_nop
% DW_CFA_nop
% \end{lstlisting}
%     \caption{The eh\_frame of function \texttt{f}.}
%     \label{fig:sub3}
%   \end{subfigure}
%   \caption{Exception handling information in an example.}
% \end{figure*}

% \begin{table}[t]
%   \caption{The format of FDE entry.}
%   \label{tab:fde}
%   \centering
%   \begin{tabular}{l p{3cm} l}
%     \hline
%     \textbf{Field}       & \textbf{Description}                & \textbf{Attribute} \\ \hline
%     Length      & Bytes of the CIE structure & Required  \\ \hline
%     CIE Pointer &                            & Required  \\ \hline
%     PC Begin & The address of the initial location of the instruction
%               related to the current FDE & Required \\ \hline
%     PC Range                 &  Number of bytes of instructions associated with this FDE  & Required        \\ \hline
%     Call Frame Instructions  &  & Required        \\ \hline
%     Extended Length          &  & \emph{Optional} \\ \hline
%     Augmentation Data Length &  & \emph{Optional} \\ \hline
%     Augmentation Data        &  & \emph{Optional} \\ \hline
%     Padding                  &  &                 \\ \hline
%   \end{tabular}
% \end{table}

\begin{lstlisting}[]
00001070 0002c 00ecc FDE cie=001a8 
pc=045fb0..045fe8
DW_CFA_advance_loc: 1 to 045fb1
DW_CFA_def_cfa_offset: 16
DW_CFA_offset: r6 (rbp) at cfa-16
DW_CFA_advance_loc: 12 to 045fbd
DW_CFA_def_cfa_offset: 24
DW_CFA_offset: r3 (rbx) at cfa-24
DW_CFA_advance_loc: 11 to 045fc8
DW_CFA_def_cfa_offset: 32
DW_CFA_advance_loc: 29 to 045fe5
DW_CFA_def_cfa_offset: 24
DW_CFA_advance_loc: 1 to 045fe6
DW_CFA_def_cfa_offset: 16
DW_CFA_advance_loc: 1 to 045fe7
DW_CFA_def_cfa_offset: 8
\end{lstlisting}

  \begin{lstlisting}[linewidth=0.9\columnwidth,breaklines=true]
000000e8 000000000000001c 00000000 CIE
  Version:               1
  Augmentation:          "zPLR"
  Code alignment factor: 1
  Data alignment factor: -8
  Return address column: 16
  Augmentation data:     9b d5 0f 20 00 1b 1b
  DW_CFA_def_cfa: r7 (rsp) ofs 8
  DW_CFA_offset: r16 (rip) at cfa-8
  DW_CFA_nop
  DW_CFA_nop

00000108 0000000000000024 00000024 FDE cie=000000e8 pc=0000000000000cdd..0000000000000dda
  Augmentation data:     b7 00 00 00
  DW_CFA_advance_loc: 1 to 0000000000000cde
  DW_CFA_def_cfa_offset: 16
  DW_CFA_offset: r6 (rbp) at cfa-16
  DW_CFA_advance_loc: 3 to 0000000000000ce1
  DW_CFA_def_cfa_register: r6 (rbp)
  DW_CFA_advance_loc: 5 to 0000000000000ce6
  DW_CFA_offset: r3 (rbx) at cfa-24
  DW_CFA_advance_loc1: 243 to 0000000000000dd9
  DW_CFA_def_cfa: r7 (rsp) ofs 8
  DW_CFA_nop
  DW_CFA_nop
  DW_CFA_nop

00000130 000000000000001c 00000104 FDE cie=00000030 pc=0000000000000dda..0000000000000e23
  DW_CFA_advance_loc: 1 to 0000000000000ddb
  DW_CFA_def_cfa_offset: 16
  DW_CFA_offset: r6 (rbp) at cfa-16
  DW_CFA_advance_loc: 3 to 0000000000000dde
  DW_CFA_def_cfa_register: r6 (rbp)
  DW_CFA_advance_loc1: 68 to 0000000000000e22
  DW_CFA_def_cfa: r7 (rsp) ofs 8
  DW_CFA_nop
  DW_CFA_nop

\end{lstlisting}


 % Line 4 in
 %  Figure~\ref{fig:sub2} advances the instruction location 1 from the
 %  function start \texttt{00000968}, so the result is \texttt{00000969}.
 %  It means the instruction location at \texttt{00000968} operates the stack.

% It is a base address in the current stack frame, which other stack
% address are calculated relatively to. An FDE includes a sequence of
% instructions record the stack change relative to the CFA.

% Typically, CFA is defined to be the value of the stack pointer at
% the call site in the previous frame (which may be different from its
% value on entry to the current frame).


% \item \texttt{DW\_CFA\_def\_cfa\_register}: define cfa register
% \item \texttt{DW\_CFA\_restore}
% \item \texttt{DW\_CFA\_def\_cfa}


A {\ehf} table contains two types of unwinding information: the
adjustment of base frame pointer and the address of callee-saved
registers. The adjustment of frame pointer is necessary for return
address calculation and address of callee-saved registers is necessary
for context restoration.

\add{(How does eh\_frame work.)}
Additionally, stack needs to be completely unwound before the program
exit. As the program continue, pop instruction on address 0xaff will
remove third records. Before the main function exit, retq instruction
will release the last record stored in the stack. 



% DWARF debug information contains separate tables for different
% debugger capabilities. In among those tables, unwind information is
% saved in .eh\_frame section.

% \textcolor{red}{ How to use unwind information.return address,
% callee saved registers(at binary address, which register, store to
% where)} Accordingly, unwinding stack is the process of removing
% function entries from function call stack. Unwinding stack is
% necessary for exception handling because normal exception handling
% but also because "forced" unwinding situations (such as unwind
% caused by longjmp or thread termination).


\add{(Explain the exception handling)}
The unwinding process begin when the program throw an exception. To
throw the exception, the program will call \texttt{<\_\_cxa\_throw@plt>}. By
searching \highlight{\_gcc\_except\_table (Where is this table? How is
  it created?)} section, \texttt{<\_\_cxa\_throw@plt>} then determine if the
current function is able to handle the exception. If the current
function fail to handle the exception, the program will trace back to
the caller function until the exception be handled. Our example
demonstrate the unwinding process as buz() function fail to handle the
exception. When program reach address \texttt{0xa9b}, program will call
\texttt{<\_\_cxa\_throw@plt>} function. The program will then return back to
main() function as throw exception failed to be handled. The searching
stage begins until the program find a proper throw exception handler.
Our program will finally find suitable throw exception handler at
address \texttt{0xae0}. As the exception be handled, the corresponding stack
records will \hl{be updated (how?)}. Before releasing the records, program
accordingly restore the register \texttt{\%rbx} value to recover the context.
The unwinding process end as the throw exception been handled.\\

% \textcolor{red}{Need a proper example to help understand how stack
% unwind works. What information eh\_frame can provide?}

% Program will walk the call stack following return address pointers to find all call frames.


% While many recursive disassemblor seeking available symbols in the
% .symtab and .dynsym sections, GHIDRA considers the .eh\_frame
% section to identify functions.


In among all the binaries, we initially analyze how much
percentage of stripped binaries included. The detailed analysis is
listed in \ref{tab:binaries}. In amount of 50 binaries, there are 4
binaries (2 open-source and 2 closed-source)that are not stripped.
Although, binary disassembling for un-stripped binary has been proved
to be un-challenging task. We consider binaries both stripped and not
stripped in our study since they both exist in real-world scenario. We
also consider binaries both PIC and none-PIC since
\textcolor{red}{explain why we expalin PIC and None-PIC}.

good answer for the first question. The result lead us to the
conclusion that eh\_frame section is commonly embodied in all kinds of
binaries (open-source \& closed-source and stripped \& not stripped).
In the following study, we limit our scope to only binaries that
contain eh\_frame section. This is reasonable because binaries missing
eh\_frame information are not only minority but also fail to follow
the x86-64 ABI rules.


% Removed from evaluation
\begin{table}[t!]
	\caption{The group of binaries our study covers}
	\label{tab:binaries}
	\centering
	\begin{tabular}{l|c|c|c|c}
		\toprule[0.5pt]
		\toprule[0.5pt]
		 \bf{\emph{Category}} & \bf{\emph{Prog-Num}} & \bf{\emph{PIC}} &\bf{\emph{Eh-frame}} &\bf{\emph{Strip}}\\ \hline
		Open-Source & 25 & 14 & 25 &23\\ \hline
		Closed-Source & 23 & 10 &23 & 21\\ 

	\bottomrule[0.5pt]
	\bottomrule[0.5pt]
	\end{tabular}
\vspace{-1.2em}
\end{table}


To answer the first question, we collected a large number of binary
programs which include 25 open-source projects and 25 closed-source
projects. The binaries we collected range from web browser, social
network program, media player, Linux tools and etc. We keep the state
of binaries without any manipulation. We believe the types of binaries
in our study represent the mainstream of widely used binary in both
research purpose and commercial purpose.


To answer the second question, we initially explain how function start
information help on binary disassembling. General disassembly
algorithms fall into two well-known categories: linear sweep and
recursive descend. Linear sweeping algorithms scan code ranges
specified by symbols in .symtab and .dynsym sections. Recursive
descend algorithms start with a given code address and follows control
flow, disassembling as it goes. Recursive descend algorithms consider
the program entry and available symbols as code addresses for
recursive disassembly. With correct symbol information, popular
disassemblors in both categories can easily achieve decent accuracy
and recall. However, binary disassembling without symbol is still a
challenge task. Without symbol information, recursive descend
algorithms ensures correctness but often result in insufficient
coverage. As aforementioned, X86-64 ABI rules mandate the unwinding
information everywhere. In fact, .eh\_frame section can be a good
substitute for symbol section to help binary disassembling. \hl{In
  .eh\_frame section, Frame Description Entry (FDE) contains Initial
  Location Field, with various bytes, to refer the initial location of
  a function. The following multiple bytes after initial location
  represent the the size of the function.} Function start and function
size are the key component for function range determination. With
complete function range information, recursive disassembling can start
from the entry point and iterate all the functions in FDEs. We design
our own .eh\_frame based binary disassemblor to further justify our
idea.
The implementation detail will be discussed in Section 4.  \\
% \textcolor{red}{More detail expalnation needed. The section question is not fully answered}\\


To answer the last and most important question, we collected various
programs as benchmarks which list in XXXXX. The programs cover
various code formats including C\&C++ code, hand-written assembly and
even hand-written binary. To further increase diversities of
evaluation, we build each program with two mainstream compilers (Gcc
and LLVM). We follow default compilation. On the other hand, past
research generally use symbol section to extract function start
information. However, such method may produce less complete ground
truth and often need human efforts. Parsing the symbol information to
determine the boundaries of function has difficulty of handling
functions with zero-size symbols. To automate full generation of
ground truth, we design a tool that intercept the end-to-end compiling
and linking process to collect ground truth, following the idea of
CCR. We then separately compare the function start information
extracted from eh\_frame with those from ground truth and symbol
section. The comparison result is shown in Table-x. When compared with
ground truth, Eh\_frame approach can achieve 99.99\% in both recall
and precision on average.


Even through function start in eh\_frame has slightly differences with those in symbol section, the minority outlayers has little influence on the overall performance.  
The promising result demonstrates that Eh\_frame section contains \highlight{almost all (?)} the function information. 
Stripping binary in fact fail to protect function information since highly similar function information can be extracted from .eh\_frame. 
To better protect stripped binary, we hereby propose a defense mechanism by re-designing exception handling.  

\subsection{Evaluation Setup}
\noindent\textbf{Benchmarks:}
We used the software listed in Table~\ref{tab:benchmarks} to experimentally
evaluate the tools we studied. The software includes programs and libraries
of diverse functionality and complexity, written in C / C++, and containing
hand-written assembly and hard-coded binary code.
% \input{tabs/benchmark.tex}


% Cut from related work
\subsection{Binary Disassembling}
Binary disassembling is a cruial task in reverse engineering and software security. There are two well-known categories of disassembly algorithms: linear sweep and recursive descend. 
The idea of linear sweeping is to continuously scan pre-selected code space and identify valid instructions. 
However, linear sweep binary disassemblor apply various mechanism on how to select sweeping ranges and how to handle errors during scanning.
OBJDUMP, as one of the most famous tool in its category, process code range specified in symbol sections.
Likewise, tools(PSI and Uroboros) following idea of OBJDUMP all start scanning from pre-selected code space based on symbol information. 
On the other hand, OBJDUMP identifies invalid opcodes as errors and keeps scanning by using heuristics.
Beyond invalid opcodes, Uroboros and PSI also handles bad opcodes and invalid control transfers.
PSI
Uroboros exclude the code around bad opcode or invalid control transfer.

As another major core algorithm in binary disassembling, recursive descend start with a given code address and follows control flow. 
The popular binary disassemblors in this category include ANGR, GHIDRA, Dyninst, Radare2.
IDA and NINJA, as commercial binary disassemblor, also apply fall into this category.  
In general, recursive descend algorithm consist of three component: (1) how to select code address, (2) how to resolve control flow, (3) how to handle the code gaps. 
Almost all the tools in this category consider program entry and available symbols as code addresses for disassembly. 
Most of the above mentioned tools determine functions by seeking available symbols in symbol section.
Function symbols are a major source of data about function entry points.
On the other hand, GHIDRA also considers the eh\_frame section to help identify functions. 
\textcolor{red}{expalin more disassembling details later.}
In summary, with symbol information, disassemblors in both categories can achieve astonishing performance in accuracy and recall. 
Without symbol information, linear sweeping disassemblors has the advantage of maximizing the recovery of instructions while hard to handle data-in-code. 
On the contrary, recursive descend disassemblors ensures correctness but often result in insufficient coverage. 
Our binary disassemblor design follow the idea of recursive descend algorithm. 
However, withour symbol information, our binary disassemblor which simply rely on function information in eh\_frame section can achieve same performance when compared with other open-sourced recursive binary disassemblor. 
More importantly, our contribution is beyond design .eh\_frame based binary disassemblor or improving binary disassembling tools. 
We aim to reveal the vulnerability of stripped binaries and re-design exception handling to better protect binaries.


The validation tool not only dynamically validate the DWARF
information, but also identify hard-to-detected bugs. In the further
step, the second tool synthesis DWARF unwind information by automatic
analysis of ELF binaries lacking unwind information.


As a X86-64 ABI requirement, Eh\_frame section has been widely applied
in ELF binary. Instead of using eh\_frame for exception handling,
\cite{oakley2011exploiting} propose an adversary aiming to take
control of the exception information. \cite{oakley2011exploiting}
claimed they could trigger a bash shell by modifying ELF binary. In
\cite{oakley2011exploiting}, to minimize the differences caused by the
modifications, modifications are limited only to eh\_frame sections
especially eh\_frame, eh\_frame\_hdr and gcc\_except\_table. The
sections including .text, .plt and etc are not allow to modify since
those sections are commonly used for insert backdoors. To solve the
difficulty of controlling parameter passing on x86-64,
\cite{oakley2011exploiting} further build a dynamic linker that locate
execvpe in libc. \cite{oakley2011exploiting} build two methods to
insert necessary data to program. The primary method is directly
writing and the second method relies on exploitation techniques to
find and overwrite memory.


==> tabs/benchmark.tex <==

\begin{table}[t!]
\scriptsize
	\centering
		\caption{Software used for evaluating tools.}
%		The list of benchmark programs used by our evaluation. \textbf{\normalsize{Prog \#}} and \textbf{\normalsize{Bin \#}} indicate the number of source-code programs and binaries, respectively (L$\shortrightarrow$Linux, W$\shortrightarrow$Windows).}
	\label{tab:benchmarks}
	 \begin{threeparttable}
%	\begin{tabular}{l|c|cc|cc}
	\begin{tabular}{l|c|c|c}
		\toprule[0.5pt]
		\toprule[0.5pt]
    
%        \multirow{2}{*}{\bf{{Type}}} &
%        \multirow{2}{*}{\bf{{Progs \& Libs}}} &
%		\multicolumn{2}{c|}{\bf{{Prog \#}}} &
%		\multicolumn{2}{c}{\bf{{Bin \#}}} \\\cline{3-6}
%		& & L & W & L & W\\ \hline
%
%		Benchmark &  SPEC CPU2006 & 30 & 15  & 546 & 120\\ \hline
%
%		Utilities  & \tabincell{c}{Unzip-6.0 Coreutils-8.30 7-zip-19\\ Findutils-4.4 Binutils-2.26 Tiff-4.0\\ } & 125 & 26 & 2500 & 196\\\hline
%		
%		Clients  & \tabincell{c}{Openssl-1.1.0l Putty-0.73 D8-6.4 \\ Filezilla-3.44.2 Busybox-1.31 \\ Protobuf-c-1 ZSH-5.7.1 VIM-8.1
%		\\ XML2-2.9.8 Openssh-8.0 Git-2.23} & 13 & 13 & 154 & 104\\\hline
%		
%		Servers  &  \tabincell{c}{Lighttpd-1.4.54 Mysqld-5.7.27 \\ Nginx-1.15.0 SQLite-3.32.0} & 3 & 2 & 49 & 16\\\hline
%
%		Libraries  & \tabincell{c}{Glibc-2.27 libpcap-1.9.0 libv8-6.4 \\ libtiff-4.0.10 libxml2-2.9.8 \\ libsqlite-3.32.0
%		libprotobuf-c-1.3.2} & 6 & 3 & 79 & 24\\\hline
%		
%		\textbf{Total}  & -- & 177 & 59 & 3328 & 460\\

        \multirow{2}{*}{\bf{{Type}}} &
        \multirow{2}{*}{\bf{{Name}}} &
		\multicolumn{2}{c}{\bf{{Programs/Binaries}}} \\
		\cline{3-4}
		& & Linux & Windows \\
		\hline

		Benchmark &  SPEC CPU2006 & 30 / 546 & 15 / 120\\
		\hline
		Utilities  & \tabincell{c}{Unzip-6.0 Coreutils-8.30 7-zip-19\\ Findutils-4.4 Binutils-2.26 Tiff-4.0\\ } & 125 / 2500 & 26 / 196 \\
		\hline
		Clients & \tabincell{c}{Openssl-1.1.0l Putty-0.73 D8-6.4 \\ Filezilla-3.44.2 Busybox-1.31 \\ Protobuf-c-1 ZSH-5.7.1 VIM-8.1
		\\ XML2-2.9.8 Openssh-8.0 Git-2.23} & 13 / 154 & 13 / 104 \\
		\hline
		Servers  &  \tabincell{c}{Lighttpd-1.4.54 Mysqld-5.7.27 \\ Nginx-1.15.0 SQLite-3.32.0} & 3 / 49 & 2 / 16 \\
		\hline
		Libraries  & \tabincell{c}{Glibc-2.27 libpcap-1.9.0 libv8-6.4 \\ libtiff-4.0.10 libxml2-2.9.8 \\ libsqlite-3.32.0
		libprotobuf-c-1.3.2} & 6 / 79 & 3 / 24 \\
		\hline
		\multicolumn{2}{l}{\textbf{Total}} & 177 / 3328 & 59 / 460 \\
	\bottomrule[0.5pt]
	\bottomrule[0.5pt]
	\end{tabular}
\vspace{-1.5em}
    \end{threeparttable}
\end{table}

==> tabs/eval-assemble-example.tex <==
\begin{figure}[ht]
  \centering
\begin{lstlisting}[language={[x86masm]Assembler},basicstyle={\footnotesize\ttfamily},numberstyle=\scriptsize,deletekeywords={df},xleftmargin=5mm]
.type   _x86_64_AES_encrypt,@function
.align  16
_x86_64_AES_encrypt:
    xorl    0(%r15),%eax
    xorl    4(%r15),%ebx
    ...
    xorl    8(%r15),%ecx
    xorl    12(%r15),%edx
.byte   0xf3,0xc3
.size   _x86_64_AES_encrypt_compact,.-_x86_64_AES_encrypt_compact
\end{lstlisting}
\caption{An assembly function from OpenSSL-1.1.0l where unwinding rules (CFIs) are not available.\label{lst:assemble_func}}
\end{figure}

==> tabs/eval-funcbody.tex <==
\begin{table}[ht]
  \centering
  
  \setlength\tabcolsep{2.3pt}
  \caption{Evaluation results of function body. The results highlighted in blue are the best results under different optimization levels.}
  \label{tab:funcbody_result}
 \begin{tabular}{l |c|c|c|c|c|c|c||c|c||c}
    \hline\hline
    \multirow{2}{*}{\textbf{OPT}}  & {\bf \angr} & {\bf \dyninst} & {\bf \ghidra} & {\bf \bap} & {\bf \radare}  & {\bf \nucleus} & {\bf \byteweight} & \multicolumn{2}{c|}{\bf \ida} & {\bf \ninja} & \multicolumn{2}{c}{\bf \tool} \\\cline{2-23}
     & P & R & P & R & P & R & P & R & P & R & P & R & P & R & P & R & P & R & P & R & P & R \\ \hline
 %   O0 & 99.98 & 99.99 & 95.40 & 99.07 & 99.92 &  97.69 &  99.94  & 99.99  &  97.14  & 91.77  & 98.92  & 97.17  &  99.96 &  97.33 & 98.82  & 99.84  & 99.30  &  98.81 & 99.63  & 99.54  & 99.99  & 99.99  \\
 %   O1 & 99.88 & 99.99 & 86.43 & 93.08 &  93.51 & 60.62  & 99.84  &  99.96 & 79.84   &  67.79 & 98.67  &  59.60 & 99.70  & 79.38  & 98.69  &  98.11 &   &   & 97.35  &  94.93 & 99.09  & 99.99  \\
    O2 & 83.66 & 95.25 &  90.85 & 63.71 &  97.13 & 99.75  & 75.29  &  54.20 &  97.47 & 50.89  &  97.79 &  90.21 & 96.38  & 96.51 & \textcolor{blue}{99.92} &  72.67 & 97.72  & 92.31 & 97.29 & \textcolor{blue}{99.99}  & 99.63  & 99.96  \\
    O3 & 83.56 & 95.63 &  90.41 & 62.09  & 96.38   &  99.78 &  73.20 &  55.55 &  97.18 & 50.61  & 97.42  &  91.98 & 97.91  &  97.75 & \textcolor{blue}{99.92}  &  75.41 & 97.63  &  94.03 & 96.52 & \textcolor{blue}{99.99} & 99.63  & 99.97  \\
    Os & 92.61 & 96.42 &  92.76 &  69.65 & 99.84  &  99.91 &  86.39 & 66.54  & 98.84  & 69.66 &  97.64 &  91.23 &  97.83 &  96.05 & 99.98 & 81.94  & 98.75  & 98.81  & 99.98  & \textcolor{blue}{99.99} & \textcolor{blue}{99.98}  & 99.96  \\
    Of & 81.89 & 95.16 &  90.71 & 62.73  &  96.56 &  99.77 & 73.58 &  56.30 & 98.14  & 50.77  & 96.00  & 91.03  &  97.02 &  96.90 & \textcolor{blue}{99.95}  & 76.19  &  97.75 & 94.22 & 96.67 & \textcolor{blue}{99.99} & 99.61  & 99.95  \\ \hline
    {\bf Avg.} & 85.43 & 95.62 &  91.18 & 64.55 & 97.48  & 99.80  & 77.12  & 58.15  & 97.92  & 55.23  & 97.21  & 91.11  & 97.29  & 96.80 & 99.94 & 85.28  & 97.84  & 94.84 & 97.62 & \textcolor{blue}{99.99}  & 99.71  & 99.96 \\\hline\hline
  \end{tabular}
\end{table}

==> tabs/eval-instructions.tex <==


\begin{table*}[ht]
  \centering
  \setlength\tabcolsep{4pt}
  \caption{Evaluation of function body detection. Best results under different optimization levels are highlighted in blue.}
  \label{tab:instresult}
  \begin{tabular}{l |c|c|c|c|c||c|c||c}
    \hline\hline
    \multirow{1}{*}{\small \textbf{OPT}}  & \multicolumn{1}{c|}{\small \bf \angr} & \multicolumn{1}{c|}{\small \bf \dyninst} & \multicolumn{1}{c|}{\bf\small  \ghidra} & \multicolumn{1}{c|}{\bf \small \bap} & \multicolumn{1}{c||}{\bf \small \radare}  & \multicolumn{1}{c|}{\bf \small \ida} & \multicolumn{1}{c||}{\small \bf \ninja} & \multicolumn{1}{c}{\small \bf \tool} \\ \hline
    O2 & 94.14 & 94.91  & 96.15 & 70.78 & 93.08 & \textcolor{blue}{99.22} & 95.48 & 98.97 \\
  O3  & 93.59 & 94.24 & 95.30  & 72.32 & 93.70 & \textcolor{blue}{99.28} & 95.53 & 98.94 \\
    Os & 94.95 & 95.83 & 96.46 & 85.86 & 94.75 & \textcolor{blue}{99.09} & 95.07 & 99.47 \\
    Of  & 93.52 & 95.07 & 95.72 & 72.31 & 94.27 & \textcolor{blue}{99.31} & 95.63 & 98.93 \\ \hline
     {\bf Avg.} & 94.05 & 95.01 & 95.91 & 75.17 & 93.95 & \textcolor{blue}{99.23} & 95.43 & 99.08 \\\hline\hline
  \end{tabular}
\end{table*}

==> tabs/eval-multi-steps.tex <==
\begin{table}[t!]
  \centering
  
%   \setlength\tabcolsep{2.3pt}
  \caption{Evaluation results of function start detection in each step of \tool. Step 1-4 respectively respond to \S~\ref{subsec:design:step1}-\ref{subsec:design:step4} (P=Precision; R=Recall).}
  \label{tab:step-by-step}
  \scriptsize
  \begin{tabular}{l |cc|cc|cc|cc}
    \hline\hline
    \multirow{2}{*}{\textbf{OPT}}  & \multicolumn{2}{c|}{\bf Step 1} & \multicolumn{2}{c|}{\bf Step 2} & \multicolumn{2}{c|}{\bf Step 3}  & \multicolumn{2}{c}{\bf Step 4} \\\cline{2-9}
     & P & R & P & R & P & R & P & R \\ \hline
    O2 & 97.28 & 99.96 & 97.28 & 99.99 &  99.96  & 99.79 & 99.96  & 99.79  \\
  O3 &  96.52 &  99.95 & 96.52 & 99.98 & 99.96  & 99.77 &  99.96 & 99.78 \\
    Os & 99.98  & 99.95 & 99.98 & 99.98  & 99.99  & 99.96 & 99.99  &  99.96 \\
    Of & 96.65 & 99.96 & 96.65 & 99.99 & 99.91  & 99.80  & 99.91  & 99.81  \\ \hline
     {\bf Avg.} & {\bf 97.61} & {\bf 99.96} & {\bf 97.61} & {\bf 99.99} & {\bf 99.96}  & {\bf 99.83} & {\bf 99.96} & {\bf 99.84} \\\hline\hline
  \end{tabular}
\end{table}

==> tabs/eval-tailcall.tex <==
\begin{table}[t!]
  \centering
  
  \setlength\tabcolsep{1.8pt}
  \caption{Evaluation results of tail call detection. The results highlighted in blue are the best results under different optimization levels (P=Precision; R=Recall).}
  \label{tab:tailcall_result}
  \scriptsize
  \begin{tabular}{l |cc|cc|cc||cc|cc||cc}
    \hline\hline
    \multirow{2}{*}{\textbf{OPT}}  & \multicolumn{2}{c|}{\bf \angr} & \multicolumn{2}{c|}{\bf \dyninst} & \multicolumn{2}{c||}{\bf \ghidra}  & \multicolumn{2}{c|}{\bf \ida} & \multicolumn{2}{c||}{\bf \textsc{Ninja}\xspace} & \multicolumn{2}{c}{\bf \tool} \\\cline{2-13}
     & P & R & P & R & P & R & P & R & P & R & P & R \\ \hline
 %   O0 & 99.98 & 99.99 & 95.40 & 99.07 & 99.92 &  97.69 &  99.94  & 99.99  &  97.14  & 91.77  & 98.92  & 97.17  &  99.96 &  97.33 & 98.82  & 99.84  & 99.30  &  98.81 & 99.63  & 99.54  & 99.99  & 99.99  \\
 %   O1 & 99.88 & 99.99 & 86.43 & 93.08 &  93.51 & 60.62  & 99.84  &  99.96 & 79.84   &  67.79 & 98.67  &  59.60 & 99.70  & 79.38  & 98.69  &  98.11 &   &   & 97.35  &  94.93 & 99.09  & 99.99  \\
    O2 & 91.95 & 78.22 & 80.67 & 77.55 &  96.76 & 98.75 & 75.09  & 80.09 & 85.40 & 97.30 & \textcolor{blue}{99.49} & \textcolor{blue}{99.68} \\
   O3 & 86.44 & 84.61  & 77.08 & 69.31 & 94.40 & 97.45 & 77.31 & 89.28 & 78.61 & 95.82 & \textcolor{blue}{99.25} & \textcolor{blue}{99.48} \\
    Os & 91.43 & 95.41  & 58.17 & 49.07 & 99.51 & 99.35 & 74.32 & 83.23 & 98.56 & 97.55 &  \textcolor{blue}{99.62} & \textcolor{blue}{99.54} \\
    Of & 86.65 & 82.72 & 77.06 & 68.15 & 94.58 & 96.80 & 77.09 & 86.54 & 79.83  & 94.38  & \textcolor{blue}{99.24} & \textcolor{blue}{99.52} \\ \hline
     {\bf Avg.} & \bf{89.12} & \bf{85.24} & \bf{73.25} & \bf{66.02} & \bf{96.31} & \bf{98.09} & \bf{75.95} & \bf{84.79} & \bf{85.60} & \bf{96.26} & \bf{\textcolor{blue}{99.40}} & \bf{\textcolor{blue}{99.56}} \\\hline\hline
  \end{tabular}
\end{table}
